Differentially-Private Clustering of Easy Instances

Clustering is a fundamental problem in data analysis. In differentially private clustering, the goal is to identify $k$ cluster centers without disclosing information on individual data points. Despite significant research progress, the problem had so far resisted practical solutions. In this work we aim at providing simple implementable differentially private clustering algorithms that provide utility when the data is "easy," e.g., when there exists a significant separation between the clusters. We propose a framework that allows us to apply non-private clustering algorithms to the easy instances and privately combine the results. We are able to get improved sample complexity bounds in some cases of Gaussian mixtures and $k$-means. We complement our theoretical analysis with an empirical evaluation on synthetic data.

==> kMeans.tex.bkp.tex <==
\section{Private $k$-Means Under Stability Assumption}\label{sec:kMeans}

In this section we present an $(\eps,\delta)$-differential private $k$-means approximation algorithm $\AlgPrivatekMeans$ with utility guarantee that holds when the input is stable in the sense that we will define. We do so by reducing the problem of approximating the $k$-means of stable data into the problem from \cref{sec:finding-averages} of approximating the averages of clusters of points that are fully-partitioned by $k$ far balls. The idea is the following: Fix a database $\cP \in (\bbR^d)^n$, a parameter $m < n$ and a (non-private) $k$-means approximation algorithm $\cA$. Now assume that when executing $\cA$ on $m$ i.i.d. samples from $\cP$, then with high probability all these sets of $k$ centers are almost located at the same positions. More formally, if we repeate the above process $T$ times (for some parameter $T$) and denote by $\tilde{C}_t = \set{\pc_1^t, \ldots, \pc_k^t}$ the centers of iteration $t \in [T]$, then our stability assumption requires that with high probability, the multiset of all resulting centers $\cC = \bigcup_{t \in [T]} \tilde{C}_t$ is fully-partitioned by $k$ far balls, where $\Partition(\cC)$ (according to \cref{def:clusters-rel}) is exactly $\set{\set{\pc_1^t}_{t=1}^T, \ldots, \set{\pc_k^t}_{t=1}^T}$ (i.e., for each $i \in [k]$, the $i$'th centers of each execution are very close to each other, compared to the distance from the other centers). Then under this assumption, \Hnote{Don't we want to formalize this assumption in some environment and give it a name/number so it is easier to refer to and the text is less vague ?} we show in this section how to use algorithm $\AlgPrivatekAverages$ for approximating the $k$-means of $\cP$. The full details of $\AlgPrivatekMeans$ are described in \cref{fig:kMeans}. The privacy guarantee is proven in \cref{sec:priv-kMeans}, the utility guarantee (under the stability assumption) is proven in \cref{sec:util-kMeans}. In \cref{sec:application} we show that a variant of the separation assumption in \cite{OstrovskyRSS12} implies our stability assumption.

%\remove{
%
%\begin{itemize}
%	\item Let $\tilde{\cC} = \emptyset$.
%	\item Repeat the following many times:
%	\begin{enumerate}
%		\item Execute $\cA$ on $m$ i.i.d. samples from $\cP$. Let $\tilde{C}$ be the output 
%	\end{enumerate}
%\end{itemize}
%
%
%Let $\cS_t$ be a database containing $m= \floor{\frac{n}{2T}}$ i.i.d. samples from $\cP$
%
%
%Now assume that $(\cP,\cA, m)$ have the property that when sampling a multiset $\cS$ which consists of $m$  i.i.d. samples from $\cP$, then the resulting centers of $\cA(\cS)$ are always belong to some fixed 
%
%
%when sampling a multiset $\cS$ of $m$ i.i.d. points from $\cP$, it holds that .... 
%
%
%we show how we can use the algorithm $\AlgPrivatekAverages$ 
%
%In this section we describe our $(\eps,\delta)$-differential private algorithm $\AlgPrivatekMeans$ that satisfies the following utility guarantee: 
%Given a multiset of points $\cP$ in $B(0,\Lambda) \subseteq \bbR^d$ which is  $(\phi,\lambda)$-separate for $k$-means (\cref{def:sep-ost}) for sufficiently small $\phi$ and some $\lambda$ to be determined by the analysis, and given a (non-private) $\omega$-approximation $k$-means algorithm $\cA$,  algorithm $\AlgPrivatekMeans$ on inputs $\cP$, $\cA$, $k$, $\beta$ outputs with probability $1-\beta$ a set of $k$ centers that $\approx (1 + O(\omega \phi^2))$-approximate the optimal $k$-means cost (plus some small additive error).
%}




\begin{figure}[thb!]
	\begin{center}
		\noindent\fbox{
			\parbox{.95\columnwidth}{
				\begin{center}{ \bf Algorithm $\AlgPrivatekMeans$}\end{center}
				\textbf{Input:} A multiset  $\cP$ of points in $B(\pt{0},\Lambda) \subseteq \bbR^d$, parameter $k \in \bbN$, privacy parameters $\eps,\delta >0$ and a confidence parameter $\beta > 0$. Let $n = \size{\cP}$.
				
				\textbf{Additional input:} A (non-private) $k$-means algorithm $\cA$.
				
				
				%. Let $n = \size{\cP}$, let $\beta \in (0,1)$ be the failure probability,  let $\eps,\delta \in (0,1)$ be the privacy parameters, and let $k \geq 2$. In addition, let $N = N(k,d,\eps,\delta)$ be a defined in \cref{sec:Strong-stab}.\Enote{We can set some lower bound on $n$, but the algorithm works properly for any $n$, except that for small values of $n$ the additive error in our guarantee will be very big compared to $n$. Think of $n >> N$}
				
				%\textbf{Additional input:} A (non-private) $k$-means algorithm $\cA$ with $(1+\alpha)$-approximation for $\phi$-separated inputs (for some $\alpha \geq 0$ and $\phi \in (0,1)$).
				\begin{enumerate}
					%\item Let $T = \ceil{N/k}$ and let $m = \floor{n/(2T)}$.
					\item Let $T \in \bbN$ be a value to be determined by the analysis.\label{step:T}
					
					\item For each $t \in [T]$:
					
					\begin{enumerate}
						\item Let $\cS_t$ be a database containing $m= \floor{\frac{n}{2T}}$ i.i.d. samples from $\cP$ (with replacement).\label{step:sample}
						
						\item Compute $\tilde{C}_t \la \cA(\cS_t)$.\label{step:non-priv-centers}
					\end{enumerate}
				
					\item Let $\tilde{\cC} = \bigcup_{t \in [T]} \tilde{C}_t$ (a ``multiset union'', that includes duplications).\label{step:new-multisets}
					
					\item Execute $\AlgPrivatekAverages$ (\cref{fig:FindAverages}) on the $kT$-size multiset $\tilde{\cC}$ with input parameters 
					
					\noindent $\tilde{\alpha} = \frac1{n}, \tilde{\eps} = \frac{\eps}{6 k}$, $\tilde{\delta} = \frac{\min\set{\delta,\beta}}{4 e^{\eps} k}$, $\tilde{k} = k$. Let $\set{\hat{\pa}_1,\ldots,\hat{\pa}_k}$ be the outcome of the execution.\label{step:the-aver-estim}
					
					\item For each $i \in [k]:$
					\begin{itemize}
						\item Let $\hat{\cP}_i$ be the points in $\cP$ that $\hpa_i$ is the closest point to them among $\set{\hat{\pa}_1,\ldots,\hat{\pa}_k}$. \label{step:compute-clusters-kmeans}
						
						\item Use the Gaussian Mechanism (\ref{fact:Gaus}) with parameters $\Lambda, \hat{\eps} = \frac{\eps}{6k}, \hat{\delta} = \frac{\delta}{8 e^{2\eps} k}, \hat{\beta} = \frac{\beta}{2k}$ to compute a noisy average $\hpc_i$ of $\hat{\cP}_i$.\label{step:add-gaus-noise}%\Enote{we need to claim that $\hat{n} = \size{\hat{\cP}_i} \geq \Omega(n/k)$}
					\end{itemize}
					
					
					\item Output $\set{\hat{\pc}_1,\ldots,\hat{\pc}_k}$.
					
					%\Enote{I removed for now the additional steps that yield approximation $(1 + \phi^2)$.}
					
%\remove{
%					\Enote{At this point we have centers that achieve constant approximation. If we want to get something like $1 + O(\phi^2)$ approximation, we need to do the following steps (see Algorithm Private-Stable-$k$-Means in the paper of Uri \& Moshe).}
%					
%					\item For each $i \in [k]$:
%					
%					\begin{itemize}
%						\item Let $\hat{D}_i = \min_{j \neq i} \norm{\pb_i - \pb_j}$.
%						
%						\item Let $\hat{\cP}_i = \set{\px \in \cP \colon \norm{\px - \pb_i} \leq \hat{D}_i/3}$.
%						
%						\item Use the Gaussian mechanism (\ref{fact:Gaus}) with privacy parameters $(\eps,\delta)$ to compute a noisy average $\hat{\pc}_i$ of $\hat{\cP}_i$. 
%					\end{itemize}
%				
%					\item Output $\hat{C} = \set{\hat{\pc}_1,\ldots,\hat{\pc}_k}$.
%}
				\end{enumerate}
		}}
	\end{center}
	\caption{A private $k$-means approximation algorithm $\AlgPrivatekMeans$ under stability assumption.\label{fig:kMeans}}
\end{figure}

\subsection{Privacy of $\AlgPrivatekMeans$}\label{sec:priv-kMeans}

The following claim states that for a suitable choice of the parameter $T$ in Step~\ref{step:T}, then the algorithm $\AlgPrivatekMeans$ is differential-private.

\begin{claim}[Privacy]\label{claim:kMeans-privacy}
	Let $N = N(d,k,\eps,\delta)= \tilde{O}\paren{k^4 d \log^4(1/\delta)/\eps^2}$ be the value from \cref{claim:main}, and assume that $T \geq \ceil{N/k}$, where $T$ is the value in Step~\ref{step:T} of $\AlgPrivatekMeans$.
	Then Algorithm $\AlgPrivatekMeans$ is $(\eps ,\delta)$-differential private.
\end{claim}
\begin{proof}
	The proof builds on the fact that switching between sampling
	with replacement and without replacement has only a small effect on
	the privacy, as stated in  \cref{fact:DP-with-replacement}.
	
	Consider a different variant of $\AlgPrivatekMeans'$, in which the sampling of the $\approx n/2$ points in all Steps~\ref{step:sample} ($m = \floor{n/(2 T)}$ points in $T$ iterations) is done without replacement. 
	Let $\cP = \set{\px_1,\ldots,\px_n}$ and $\cP' = \set{\px_1',\ldots,\px_n'}$ be two neighboring databases of points \Enote{define}. In the following we consider two independent executions $\AlgPrivatekMeans'(\cP)$ and $\AlgPrivatekMeans'(\cP')$ (both with the same parameters $k,\eps,\delta,\beta$). In the execution $\AlgPrivatekMeans'(\cP)$, for $t \in [T]$ let $\cJ_t \subseteq [n]$ be the $m$ chosen indices of the points $\cS_t$ in Step~\ref{step:sample} (i.e., $\cS_t = \set{\px_j}_{j \in \cJ_t}$), and let $\cJ_t'$ be the indices w.r.t the execution $\AlgPrivatekMeans'(\cP')$. Since $\cJ_t$ and $\cJ_t'$ only depend on $n$ and not on the content of $\cP$ and $\cP'$, it is enough to prove that the output of both executions is $(\eps,\delta)$-indistinguishable conditioned on the event that $\cJ_t = \cJ_t'$ for every $t \in [T]$. In the following, we assume that this event occurs.
	Since $\cP$ and $\cP'$ are neighboring, there exists at most one index $t \in [T]$ such that $\cS_t$ of the execution $\AlgPrivatekMeans'(\cP)$ is different than the corresponding set in $\AlgPrivatekMeans'(\cP')$, and therefore, the resulting $\hat{\cC}$ in Step~\ref{step:new-multisets} is different by at most $k$ points. Since $\AlgPrivatekAverages$ is $(\tilde{\eps},\tilde{\delta})$-differential private for multisets of size $\geq N$ (\cref{claim:privacy}), we deduce that the resulting $k$ averages $\set{\tpa_1,\ldots,\tpa_k}$ in Step~\ref{step:the-aver-estim} are $(k\tilde{\eps},k\tilde{\delta})$- indistinguishable, i.e., Step~\ref{step:the-aver-estim} is $(\frac{\eps}{6}, \frac{\delta}{4 e^{\eps}})$-differential private. Note that for any fixing of $\set{\tpa_1,\ldots,\tpa_k}$, Step~\ref{step:add-gaus-noise} is a composition of $k$ Gaussian mechanisms, and by basic composition (\cref{thm:composition1}) it is $(\frac{\eps}{6}, \frac{\delta}{8 e^{2\eps}})$-differential private. By iterative composition \Enote{is iterative is the right word?} of Step~\ref{step:the-aver-estim} and Step~\ref{step:add-gaus-noise} (\cref{fact:iter-comp}), we deduce that $\AlgPrivatekMeans'$ is $(\frac{\eps}{3}, \frac{\delta}{2 e^{\eps}})$-differential private. Finally, we conclude that the original $\AlgPrivatekMeans$, that chooses the points with replacement, is $(\eps,\delta)$-differential private by applying \cref{fact:DP-with-replacement} with $m = n/2, \frac{\eps}{3}, \frac{\delta}{2 e^{\eps}}$.
\end{proof}


%Before stating our utility guarantee, we first start with some definitions of events and claims about them.

%\subsection{Events and Facts over the Execution of $\AlgPrivatekMeans$}

%\subsubsection{Events and Facts from Uri and Moshe's paper}

\subsection{Utility of $\AlgPrivatekMeans$}\label{sec:util-kMeans}

\Enote{Continue from here}
In the following, we formalize our stability assumption by fixing some arbitrary set of $k$ centers $C= \set{\pc_1,\ldots,\pc_k}$ and a parameter $\gamma \in [0,1]$ and require that all resulting centers $\tilde{C}_t$ in Step~\ref{step:non-priv-centers} are "$\gamma$-close" to $C$: 


%In this section we focus on proving the utility guarantee of $\AlgPrivatekMeans$. Towards this goal, in this section we fix the inputs $\cP,k,\eps,\delta,\beta,\cA$ for $\AlgPrivatekMeans$, where we assume that $\cA$ is an $\omega$-approximation algorithm for $k$-means, and we consider a random execution of $\AlgPrivatekMeans$ over these values.


\begin{definition}[Event $E_{C}^{\gamma}$ (over a random execution of $\AlgPrivatekMeans$)]\label{def:event-ECgamma}
	Let $\gamma \in [0,1]$, $C = \set{\pc_1,\ldots,\pc_k} \subseteq \bbR^d$ and let $D_i = \min_{j \neq i}\norm{\pc_i - \pc_j}$. We define $E_{C}^{\gamma}$ to be the event that for every $t \in [T]$ and $i \in [k]$, there exists $\tpc_i^t \in \tilde{C}_t$  such that $\norm{\tpc_i^t - \pc_i} \leq \gamma\cdot D_i$.
\end{definition}

Assuming that for each $i \in [k]$ the centers $\set{\pc_i^t}_{t=1}^T$ are close to each other, then for each $i$ any choice of a point $\pc_i$ that is close to $\set{\pc_i^t}_{t=1}^T$ will make the event $E_{C}^{\gamma}$ to occur (for suitable $\gamma$). Therefore, we can think of $C = \set{\pc_1,\ldots,\pc_k}$ as the choice of such centers that minimize $\COST_{\cP}(C)$. If $\cA$ is an $\omega$-approximation algorithm for $k$-means, it holds that $\COST_{\cP}(C) \leq \min\set{\COST_{\cP}(\tilde{C}_t)}_{t=1}^T \approx \min\set{ \omega \cdot \OPT_k(\cP)}_{t=1}^T$ (the ``$\approx$'' holds by \cref{prop:cost-of-sample-is-good} for large enough $m$). In \cref{sec:application} we even see that when $\cP$ is separated for $k$-means according to \cite{OstrovskyRSS12}, then with high probability the event $E_{C^*}^{\gamma}$ occur, where $C^*$ is an optimal $k$-means for $\cP$.

The following lemma summarizes the utility guarantee of $\AlgPrivatekMeans$. Roughly speaking, the lemma states that when event $E_{C}^{\gamma}$ occurs, then with high probability $\AlgPrivatekMeans$ outputs $k$ centers $\hat{C} = \set{\hat{\pc}_1,\ldots,\hat{\pc}_k}$ such that $\COST_{\cP}(\hat{C})$ is bounded by $(1 + O(\gamma)) \COST_{\cP}(C)$ (plus some small additive error).

\begin{lemma}[Utility]\label{lem:kMeans-utility}
	Let $\eps,\delta,\beta \in (0,1)$, let $\cA$ be a (non-private) algorithm, let $\cP \in (B(\pt{0},\Lambda))^n$, let $C = \set{\pc_1,\ldots,\pc_k} \subseteq \bbR^d$ with $\min_{i \neq j} \norm{\pc_i - \pc_j} \geq 1/n$ and let $\gamma \in [0,\frac1{28})$. Consider a random execution of $\AlgPrivatekMeans$ on inputs $\cP,k,\eps,\delta,\beta,\cA$ with 
	\begin{align*}
		T = \Omega\paren{\frac{d k^2 \ell \sqrt{\log\paren{\frac{k \ell}{\min\set{\beta,\delta}}}}}{\gamma} \cdot \log\paren{\frac{d k \ell n \Lambda}{\min\set{\beta,\delta}}}},
	\end{align*}
	letting $\ell = \tilde{O}\paren{(dk \log(T/\delta) + \log^2(1/\delta))/\eps}$ be the value from \cref{claim:main} with respect to $\tilde{n} = k T, d, k, \tilde{\eps} = \frac{\eps}k, \tilde{\delta} = \frac{\min\set{\delta,\beta}}{k}$.
	Assume that event $E_{C}^{\gamma}$ occurs, and let  $\hat{C} = \set{\hpc_1,\ldots,\hpc_k}$ be output of the execution. Then with probability $1-\beta/2$ it holds that
	\begin{align*}
		COST_{\cP}(\set{\hpc_1,\ldots,\hpc_k}) \leq (1 + 64\gamma) \COST_{\cP}(C) +  O\paren{\frac{\Lambda^2 k^4 d}{\eps^2}  \log(k/\delta) \log(k/\beta)}
	\end{align*}
\end{lemma}

\begin{proof}
	In the following, for $t \in [T]$ let $\hat{C}_t = \set{\hpc_1^t,\ldots,\hpc_k^t}$ where we denote by $\hpc_i^t$ the center that is close to $\pc_i$, i.e., $\norm{\hpc_i^t - \pc_i} \leq \gamma \cdot D_i$, where $D_i = \min_{j \neq i}\norm{\pc_i- \pc_j}$ (holds by event $E_C^{\gamma}$). In addition, for $i \in [k]$, let $\pa_i = \Avg(\set{\hpc_{i}^t}_{t=1}^T)$ and note that
	\begin{align}\label{eq:dist-pai-pci}
		\forall i \in [k]:\text{}\norm{\pa_i - \pc_i} \leq \gamma \cdot D_i
	\end{align}
	Now, let $\cC$ be the multiset from Step~\ref{step:new-multisets} of the algorithm, and note that $\cC$ is fully-partitioned by the set of balls $\set{B(\pc_i, r_i = 2\gamma D_i)}_{i=1}^k$ which are also \textbf{very} far balls (according to \cref{def:sep-balls}) since $\gamma < \frac1{28}$, and the clusters of $\cC$ are $\set{\set{\hpc_{1}^t}_{t=1}^T, \ldots, \set{\hpc_{k}^t}_{t=1}^T}$. Therefore, when applying algorithm $\AlgPrivatekAverages$ in Step~\ref{step:the-aver-estim}, we obtain by \cref{claim:utility-kAverg} a set of $k$ points $\set{\hpa_1,\ldots,\hpa_k}$ such that
	\begin{align}\label{eq:dist-pai-hpai}
		\forall i \in [k]:\text{   }
		&\text{}\norm{\pa_i - \hpa_i}\nonumber\\
		&\leq  O\paren{\frac{r_i \cdot d k^2 \ell \sqrt{\log(k \ell/\tilde{\delta})}}{\tilde{\eps} \tilde{n}} \paren{(1 + \tilde{\alpha}/r_i) \log(d k \ell/\tilde{\delta}) + \log \paren{\frac{\Lambda d k}{\tilde{\alpha} \tilde{\delta}}}}}\nonumber\\
		&\leq O\paren{\frac{d k^2 \ell \sqrt{\log\paren{\frac{k \ell}{\min\set{\beta,\delta}}}}}{T} \cdot \log\paren{\frac{d k \ell n \Lambda}{\min\set{\beta,\delta}}}} \cdot D_i\\
		&\leq \gamma\cdot D_i,\nonumber
	\end{align}
	where in the second inequality we used the fact that $r_i \leq D_i$ and that $D_i \geq 1/n = \tilde{\alpha}$, and in the second inequality we used the lower bound on $T$. Therefore, we deduce by \cref{eq:dist-pai-pci,eq:dist-pai-hpai} that 
	\begin{align}
		\forall i \in [k]:\text{}\norm{\hpa_i - \pc_i} \leq 2\gamma \cdot D_i
	\end{align}
	Now, let $\hat{\cP}_1,\ldots,\hat{\cP}_k$ be the clusters from Step~\ref{step:compute-clusters-kmeans} of the algorithm. By \cref{prop:close-centers-have-similar-cost} we get that 
	\begin{align}\label{eq:avg-cost}
		\sum_{i=1}^k \sum_{\px \in \hat{\cP}_i} \norm{\px - \Avg(\hat{\cP}_i)}^2 \leq (1 + 64\gamma) \COST_{\cP}(C) 
	\end{align}
	Since the algorithm compute a noisy estimation $\hpc_i$ of each $\Avg(\hat{\cP}_i)$, we get by the properties of the Gaussian mechanism (see \cref{obs:Gaus-aver}) that with probability $1-\beta$ it holds that
	\begin{align}\label{eq:dist-from-avg}
		\forall i \in [k]:\text{}\norm{\hpc_i - \Avg(\hat{\cP}_i)} 
		&\leq O\paren{\frac{\Lambda}{\hat{\eps} \size{\hat{\cP}_i}} \sqrt{d \log(1/\hat{\delta}) \log(1/\hat{\beta})}}\\
		&= O\paren{\frac{\Lambda k^2}{\eps \size{\hat{\cP}_i}} \sqrt{d \log(k/\delta) \log(k/\beta)}}\nonumber
	\end{align}
	We conclude from \cref{eq:avg-cost,eq:dist-from-avg} that 
	\begin{align*}
		\lefteqn{\COST_{\cP}(\set{\hpc_1,\ldots,\hpc_k})}\\
		&\leq \sum_{i=1}^k \sum_{\px \in \hat{\cP}_i} \norm{\px - \hpc_i}^2\\
		&= \sum_{i=1}^k \sum_{\px \in \hat{\cP}_i} \paren{\norm{\px - \Avg(\hat{\cP}_i)}^2 + \norm{\hpc_i - \Avg(\hat{\cP}_i)}^2 + 2 \norm{\px - \Avg(\hat{\cP}_i)}\cdot \norm{\hpc_i - \Avg(\hat{\cP}_i)}}\\
		&\leq (1 + 64\gamma) \COST_{\cP}(C) + O\paren{\frac{\Lambda^2 k^4 d}{\eps^2}  \log(k/\delta) \log(k/\beta)} + 2 \Delta \cdot O\paren{\frac{\Lambda k^3}{\eps} \sqrt{d \log(k/\delta) \log(k/\beta)}}\\
		&= (1 + 64\gamma) \COST_{\cP}(C)  + O\paren{\frac{\Lambda^2 k^4 d}{\eps^2}  \log(k/\delta) \log(k/\beta)}
	\end{align*}
\end{proof}



\remove{

%\begin{definition}[The additive separation error $\lambda$]\label{def:lambda}
	%Let $\lambda_k \eqdef \max_{t \in [T]} \set{\Delta(\tilde{C}_t)}|_{E_1}$, let $\lambda_{k-1} \eqdef \max_{t \in [T]} \set{\Delta(C^{*k-1}_{\cS_t})}|_{E_1}$ (i.e., a bound on these values when $E_1$ occurs), and let 
	
	%\begin{align*}
	%	\lambda \eqdef 2(\lambda_k + \phi^2 \lambda_{k-1}) \leq 2(1 + \phi^2) \sqrt{M \Lambda^2 n} \approx \sqrt{n \log(n)} \cdot \sqrt{\Lambda^4 N d \cdot  \ln \paren{\frac{d N}{\beta k}}}
	%\end{align*}
%\end{definition}

%\begin{fact}\label{fact:simple-sep-fact}
%	For $\lambda = \lambda_k + \phi^2 \lambda_{k-1}$, it holds that $$\OPT_{k}(\cP) + \lambda \leq \phi^2 \OPT_{k-1}(\cP) \iff \frac{\OPT_{k}(\cP) + \lambda_k}{\OPT_{k-1}(\cP) - \lambda_{k-1}} \leq \phi^2$$.
%\end{fact}
}


%\Enote{Actually, we only need $\lambda$ to be a bound on $\max_{t \in [T]} \set{\Delta(\tilde{C}_t), \Delta(C^{*k-1}_{\cS_t})}$ that holds w.h.p. Can we bound it in terms of $\Delta(C^{* k}_{\cP}) \approx \sqrt{M \cdot \OPT_k(\cP)}$ and $\Delta(C^{* k-1}_{\cP})\approx \sqrt{M \cdot \OPT_{k-1}(\cP)}$?}

%\Enote{Can we set $\lambda$ to be $\Delta(C_{\cP}^{* k})$ or $\Delta(C_{\cP}^{*k-1})$? I don't see how, so this is a disadvantage of this approach compared to lower-bounding $\OPT_k(\cP)$ approach, since in any case we need to pay an additive error of $\approx \sqrt{n}$. See the next claim}

%\Enote{
%\begin{definition}[The additive separation error $\lambda$]
%		\begin{align*}
%			\lambda \eqdef n \cdot (\Delta(C^{* k}_{\cP}) + \phi^2 \Delta(C^{* k-1}_{\cP}))
%		\end{align*}
		%\Enote{For $\lambda = \lambda' + \phi^2 \lambda''$, note that $\OPT_{k}(\cP) + \lambda \leq \phi^2 \OPT_{k-1}(\cP) \iff \frac{\OPT_{k}(\cP) + \lambda'}{\OPT_{k-1}(\cP) - \lambda''} \leq \phi^2$}
%\end{definition}
%}

\remove{
%\begin{claim}[Event $E_6$]\label{claim:E_6}
%	\Enote{I think we don't need this event anymore:}Let $E_6$ be the event that for every $t \in [T]$, the multiset $\cS_t$ is $\phi$-separated. Then, if $\cP$ is $(\phi,\lambda)$-separated, it holds that $E_1 \subseteq E_6$.
%\end{claim}
%\begin{proof}
%	Assume that event $E_1$ occurs, and fix $t \in [T]$.  Let $C^{*k}_{\cP}$ be the optimal set of $k$ centers for $\cP$. Similarly, let $C^{*k-1}_{\cP}$, $C^{*k}_{\cS_t}$, $C^{*k-1}_{\cS_t}$. The proof follows by the following calculation
%	\begin{align*}
%		\frac{\OPT_k(\cS_t)}{\OPT_{k-1}(\cS_t)} 
%		&= \frac{\frac{n}m \cdot \COST_{\cS_t}(C^{*k}_{\cS_t})}{\frac{n}m \cdot \COST_{\cS_t}(C^{*k-1}_{\cS_t})}\\
%		&\leq \frac{\frac{n}m \cdot \COST_{\cS_t}(C^{*k}_{\cP})}{\frac{n}m \cdot \COST_{\cS_t}(C^{*k-1}_{\cS_t})}\\
%		&\leq \frac{\COST_{\cP}(C^{*k}_{\cP}) + \Delta(C^{*k}_{\cP})}{\COST_{\cP}(C^{*k-1}_{\cS_t}) - \Delta(C^{*k-1}_{\cS_t})}\\
%		&\leq \frac{\OPT_k(\cP)+ \lambda_k}{\OPT_{k-1}(\cP) - \lambda_{k-1}}\\
%		&\leq \phi^2,
%	\end{align*}
%	where the last inequality holds by \cref{fact:simple-sep-fact}.
	%where the third inequality holds whenever $\OPT_{k-1}(\cP) \geq M/4$ since the function $f(x) = x - \sqrt{M x}$ is increasing in the range $[M/4,\infty)$.
%\end{proof}
}


\remove{
\Enote{Delete the following event}

%\begin{corollary}[Event $E_5$]\label{cor:E_5}
%	Fix some (non private) algorithm $\cA$ for $k$-means with $c$-approximation for $2\phi$-separated inputs.  For every $t \in [T]$, let $\tilde{C}^t = (\tpc_1^t,\ldots,\tpc_k^t) = \cA(\cS_t)$. Let $E_5$ be the event that there exists a permutation $\pi$ of $[k]$ such that for all $i \in [k]$ it holds that $\norm{\pc_i^* - \tpc_{\pi(i)}^t} \leq D_i/4$. Assuming that: (1) $\cP$ is $\phi$-separated for $k$-means, and that (2) $\OPT_k(\cP) > 100 \cdot \max\set{1, \frac{16 \phi^2}{1 - \phi^2}} \cdot \frac{\Lambda^2 n k d}{m} \cdot \ln \paren{\frac{2ndT}{\beta}}$, and that (3) $\max\set{\frac{\alpha + 4\phi^2}{1-4\phi^2},\frac{\alpha + 2\phi}{1-2\phi}} < \frac1{16}$ for $\alpha = 4 c \phi^2$. Then 
%	it holds that $\pr{E_5} \geq 1-\beta$.
%\end{corollary}
%\begin{proof}
%	Assume that events $E_1$ holds, and therefore $E_6 \land E_3$ hold (by \cref{claim:E_6,claim:E_3}. Since $\cS_t$ is $2\phi$-separated (by event $E_6$), and since $\COST_{\cS_t}(\tilde{C}^t) \leq c \cdot \OPT_k(\cS_t) \leq \alpha \cdot \OPT_{k-1}(\cS_t)$, we can apply \cref{thm:Ostrovsky} on $C^t$ and $\tilde{C}^t$ to obtain that there exists a permutation $\pi'$ of $[k]$ such that for all $i \in [k]$ it holds that $\norm{\pc_i^t - \tpc_{\pi'(i)}^t} \leq D_i/8$. By event $E_3$,  there exists a permutation $\pi''$ of $[k]$ such that for all $i \in [k]$ it holds that $\norm{\pc_i^* - \pc_{\pi''(i)}^t} \leq D_i/8$. By combining the two results we deduce that the permutation $\pi = \pi' \circ \pi''$ satisfies for all $i \in [k]$ that $$\norm{\pc_i^* - \tpc_{\pi(i)}^t} \leq \norm{\pc_i^* - \pc_{\pi''(i)}^t} + \norm{\pc_{\pi''(i)}^t - \tpc_{\pi' (\pi''(i))}^t} \leq D_i/8 + \min_j\set{D_j}/8 \leq D_i/4$$
%	Therefore, we deduce that $E_1 \subseteq E_5$, and using \cref{claim:E_1}, we deduce that $\pr{E_5} \geq \pr{E_1} \geq 1-\beta$.
%\end{proof}
}


